Multiobjective Tactical Planning under Uncertainty for Air Traffic Flow and Capacity Management

We investigate a method to deal with congestion of sectors and delays in the tactical phase of air traffic flow and capacity management. It relies on temporal objectives given for every point of the flight plans and shared among the controllers in order to create a collaborative environment. This would enhance the transition from the network view of the flow management to the local view of air traffic control. Uncertainty is modeled at the trajectory level with temporal information on the boundary points of the crossed sectors and then, we infer the probabilistic occupancy count. Therefore, we can model the accuracy of the trajectory prediction in the optimization process in order to fix some safety margins. On the one hand, more accurate is our prediction; more efficient will be the proposed solutions, because of the tighter safety margins. On the other hand, when uncertainty is not negligible, the proposed solutions will be more robust to disruptions. Furthermore, a multiobjective algorithm is used to find the tradeoff between the delays and congestion, which are antagonist in airspace with high traffic density. The flow management position can choose manually, or automatically with a preference-based algorithm, the adequate solution. This method is tested against two instances, one with 10 flights and 5 sectors and one with 300 flights and 16 sectors.

==> instance.tex <==
\begin{figure}
  \centerline{
    \begin{tikzpicture}
      [scale=0.5,every node/.style={circle,fill=green!20,scale=0.5}]
      \node (n1) at (-4,4) {$X_1$};
      \node (n2) at (-4,2)  {$X_2$};
      \node (n3) at (-4,0) {$X_3$};
      \node (n4) at (-4,-2) {$X_4$};
      \node (n5) at (-4,-4) {$X_5$};
      \node (n6) at (4,4)  {$X_6$};
      \node (n7) at (4,2) {$X_7$};
      \node (n8) at (4,0) {$X_8$};
      \node (n9) at (4,-2) {$X_9$};
      \node (n10) at (4,-4) {$X_{10}$};
      \node (n11) at (-2,2)  {$X_{11}$};
      \node (n12) at (-2,-2) {$X_{12}$};
      \node (n13) at (2,2) {$X_{13}$};
      \node (n14) at (2,-2) {$X_{14}$};
      \node (d1) at (-6,4) {$D_1$};
      \node (d2) at (-6,2) {$D_2$};
      \node (d3) at (-6,0) {$D_3$};
      \node (d4) at (-6,-2) {$D_4$};
      \node (d5) at (-6,-4) {$D_5$};
      \node (d6) at (6,4) {$D_6$};
      \node (d7) at (6,2) {$D_7$};
      \node (d8) at (6,0) {$D_8$};
      \node (d9) at (6,-2) {$D_9$};
      \node (d10) at (6,-4) {$D_{10}$};
      \draw[-] (d1) edge (n1);
      \draw[-] (d2) edge (n2);
      \draw[-] (d3) edge (n3);
      \draw[-] (d4) edge (n4);
      \draw[-] (d5) edge (n5);
      \draw[-] (d6) edge (n6);
      \draw[-] (d7) edge (n7);
      \draw[-] (d8) edge (n8);
      \draw[-] (d9) edge (n9);
      \draw[-] (d10) edge (n10);
      \draw[-] (n1) edge (n11);
      \draw[-] (n2) edge (n11);
      \draw[-] (n3) edge (n11);
      \draw[-] (n4) edge (n12);
      \draw[-] (n5) edge (n12);
      \draw[-] (n6) edge (n13);
      \draw[-] (n7) edge (n13);
      \draw[-] (n8) edge (n14);
      \draw[-] (n9) edge (n14);
      \draw[-] (n10) edge (n14);
      \draw[-] (n13) edge (n14);
      \draw[-] (n11) edge (n14);
      \draw[-] (n12) edge (n13);
      \begin{pgfonlayer}{background}
%\filldraw[fill=red!20,snake=bumps] (0,0) rectangle (3,2);
        \filldraw [fill=red!30,draw=red]
        (n12.east) rectangle (n13.west);
        \filldraw [fill=red!30,draw=red]
        (n3.east) rectangle (n1.east -| n11.west);
        \filldraw [fill=red!30,draw=red]
        (n5.east) rectangle (n4.north -| n12.west);
        \filldraw [fill=red!30,draw=red]
        (n13.south -| n13.east) rectangle (n6.west);
        \filldraw [fill=red!30,draw=red]
        (n8.east -| n14.east) rectangle (n10.west);
      \end{pgfonlayer}
    \end{tikzpicture}
  }
  \caption{\label{fig:inst}The 10-flights-and-5-sectors instance}
\end{figure}

